Sequence Transferability and Task Order Selection in Continual Learning

In continual learning, understanding the properties of task sequences and their relationships to model performance is important for developing advanced algorithms with better accuracy. However, efforts in this direction remain underdeveloped despite encouraging progress in methodology development. In this work, we investigate the impacts of sequence transferability on continual learning and propose two novel measures that capture the total transferability of a task sequence, either in the forward or backward direction. Based on the empirical properties of these measures, we then develop a new method for the task order selection problem in continual learning. Our method can be shown to offer a better performance than the conventional strategy of random task selection.

==> table_iclr/table_correlation_no_buffer.tex <==
\begin{table*}[ht]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{cccc}
\hline
Dataset         & Method/Buffer & Total Forward Transferability & Total Reverse Transferability \\ \hline
Split CIFAR-10  & LWF           & $0.28^{\dagger}$              & $0.19^{\dagger}$              \\
                & SI            & $0.10^{\dagger}$                        & $\mathbf{0.15^{\dagger}}$               \\ \hline
Split CIFAR-100 & LWF           & $0.14^{\dagger}$             & $\mathbf{0.28^{\dagger}}$     \\
                & SI            & $0.47$                        & $\mathbf{0.57}$              
\end{tabular}
% }
\par{\text{}}
% \par{\text{}}
\caption{Pearson correlation coefficients between AA, TFT and TRT after training. The symbol $\dagger$ denotes that the corresponding value is not statistical significant ($p\geq0.05$). Bold values indicate that TRT has higher correlations with AA than TFT.}
\vspace*{-0.1in}
\label{table:correlation:no_buffer}
\end{table*}
